A Paradigm For Collaborative Pervasive Fog Computing Ecosystems at the Network Edge

While the success of edge and fog computing increased with the proliferation of the Internet of Things (IoT) solutions, such novel computing paradigm, that moves compute resources closer to the source of data and services, must address many challenges such as reducing communication overhead to/from datacenters, the latency to compute and receive results, as well as energy consumption at the mobile and IoT devices. fog-to-fog (f2f) cooperation has recently been proposed to increase the computation capacity at the network edge through cooperation across multiple stakeholders. In this paper we adopt an analytical approach to studying f2f cooperation paradigm. We highlight the benefits of using such new paradigm in comparison with traditional three-tier fog computing paradigms. We use a Continuous Time Markov Chain (CTMC) model for the N f2f cooperating nodes and cast cooperation as an optimization problem, which we solve using the proposed model.

==> MarckovOld.tex <==
 In this case, to determine the set of loads for which cooperation is convenient, we can use the Erlang-B formula that for just one or two servers is $\frac{\la a_2 = \pi_{01} p_1 \lambda_2mbda}{1+\lambda}$ and $\frac{\lambda^2}{2+2\lambda+\lambda^2}$ respectively. Assuming $\lambda_1 > \lambda_2$, for cooperation to be convenient for both nodes, it must be:
$$
\frac{(\lambda_1+\lambda_2)^2}{2+2(\lambda_1+\lambda_2)+(\lambda_1+\lambda_2)^2} < \frac{\lambda_2}{1+\lambda_2}
$$ 
After some manipulation one finds the critical value indicating the minimum $\lambda_2$ for which cooperation is convenient: (see also Figure \ref{fig:CONV})
\begin{equation}
\lambda_2 > \lambda^c_1 = \sqrt{1+\lambda_1}-1
\label{equ:LOAD_CONV}
\end{equation}

\begin{figure}[ht] 
    \centering
  \includegraphics[width=0.48\linewidth]{eps/cross} 
    %\vspace{4ex}
\caption{Cooperation convenience}
\label{fig:CONV} 
\end{figure}%% 

As role of thumb $\lambda^c=\frac{\lambda}{2}. $We now will show that when nodes cooperate with a certain probability, cooperation can be made convenient for arbitrary loads. Before that, it is worth to analyze why use probability at all.
Deterministic rules to regulate cooperation fail


To understand the effect of the cooperation probabilities, Figure \ref{fig:PARETO_095095} shows $b_1()$ and $b_2()$ for $\lambda_1=\lambda_2=0.95$ as a function of the cooperation probabilities and two contour lines on the $p_1 \times p_2$ domain, one for $b_1(p_1,p_2)=b_1(0,0)$ (bottom line) and the other for $b_2(p_1,p_2)=b_2(0,0)$, that divide the domain $[0,1]^2$ into two parts. A domain $P$ where the blocking probability is lower the two nodes at the same time, labelled OK, and the remaining part where one of the two nodes has a higher blocking probability. The two arrows point to the direction where the decrease in the blocking probability is maximum, see later.
\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering    \includegraphics[width=0.99\linewidth]{eps/pareto12_095095}
    \label{fig:P12_095}
    \caption{Cooperation probability effect}
    %\vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso095095}       
  \caption{Cooperation domains}
  \label{fig:DOMAIN_095095} 
  \end{subfigure}
\caption{Blocking probabilities vs cooperation probabilities, for $\lambda_1=\lambda_2=0.95$}
\label{fig:PARETO_095095}
\end{figure}
The next two figures show that $P$, when $\lambda_2<\lambda_1$ is not empty and, in particular, this also occurs when loads violate the condition expressed by Equation \ref{equ:LOAD_CONV}. Figure \ref{fig:PARETO_09504} shows the blocking probabilities and cooperation domains for $\lambda_1=0.4,\lambda_2=0.95,$, i.e., $\lambda_2>\sqrt{\lambda_1+1}-1$, whereas Figure for $\lambda_1=0.4,\lambda_2=0.25,$, i.e., $\lambda_2<\sqrt{\lambda_1+1}-1$

\begin{figure}[ht] 
  \centering
    \begin{subfigure}[b]{0.5\linewidth}
  \includegraphics[width=0.99\linewidth]{eps/pareto12_09504} 
    \caption{Blocking probabilities} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso09504}
    \caption{Cooperation domains} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
    \caption{Blocking probabilities for $\lambda_1=0.95,\lambda_2=0.4$}
    \label{fig:PARETO_09504} 
\end{figure}


\begin{figure}[ht] 
  \centering
    \begin{subfigure}[b]{0.5\linewidth}
  \includegraphics[width=0.99\linewidth]{eps/pareto12_095025} 
    \caption{Blocking probabilities} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso095025}
    \caption{Cooperation domains} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
    \caption{Blocking probabilities for $\lambda_1=0.95,\lambda_2=0.25$}
    \label{fig:PARETO_095025} 
\end{figure}

\subsection{Optimum way to cooperate} Q2) Is there exits a cooperation probability pair that minimizes the blocking probabilities for both nodes? To answer to this question, it is useful to first considering the problem of minimizing the blocking probabilities as a multi-objectives minimization problem 
$$
min [b_1(\mathbf{p}),b_2(\mathbf{p})] \:\:\:\: \mathbf{p} \in [0,1]^2
$$
where $\mathbf{p}=(p_1,p_2)$. Note that in our problem we additional require that $b_1(\mathbf{p})<b_1(0),b_2(\mathbf{p})<b_2(0)$.

We can now use the notion of Pareto efficiency. For a given a cooperation probability pair, $\mathbf{p}$, $\mathbf{p}'$ is a Pareto improvement wrt $\mathbf{p}$, if $b_1(\mathbf{p}')<b_1(\mathbf{p})$ and $b_2(\mathbf{p}') \leq b_2(\mathbf{p})$ or $b_2(\mathbf{p}')<b_2(\mathbf{p})$ and $b_1(\mathbf{p}') \leq b_1(\mathbf{p})$, i.e., with the new solution at least one blocking probability is lower than the old one. Also, $\mathbf{p}^*$ is said to be Pareto efficient (or optimal) if it doesn't exit any Pareto improvement   wrt to $\mathbf{p}^*$. The set of pairs that are Pareto optimal is called the set of efficient solutions, $\partial P$, and the corresponding  image through the $\mathbf{b}=(b_1,b_2)$  function, the Pareto frontier, $\partial B$, i.e., $\partial B = \mathbf{b}(\partial P)$. So the answer to the original question is that the optimal cooperation probability pair is any pair in the $\partial P$ set and such that $b_1(\mathbf{p})<b_1(0),b_2(\mathbf{p})<b_2(0)$%As we also want that for the two nodes the blocking probability under cooperation should be less than they do not cooperate
Figure \ref{fig:IMAGE} shows an example of the Pareto frontier for $\lambda_1=\lambda_2=0.95$. 


\begin{figure}[ht] 
\centering
  \includegraphics[width=0.7\linewidth]{eps/image} 
    \label{fig:IMAGE} 
    \caption{An example of Image of the b function for $\lambda_1=\lambda_2=0.9$. The two solid lines is the (convenient) Pareto frontier; dashed lines represent the border after which cooperation is not convenient for one of the two nodes.} 
    \label{fig:FRONTIERA} 
\end{figure}




\subsection{Reaching optimum cooperation} Q3) How the two nodes can agree on determining such optimal cooperation probabilities using a distributed algorithm? First of all, we know that there are many Pareto efficient probability cooperation pairs, and that, assuming $\lambda_2 < \lambda_1$, their form is $(1,p_2)$, with $p_2 \le 1$. In principle, any of them is a convenient choice. However, an additional reasonable criteria to seek among these probabilities is to require that the rate at which $n_1$ borrows its server to $n_2$ is to be equal to the rate at which $n_2$ borrows its server to $n_1$. We call this requirement {\it fair} cooperation. Although convenient wrt to cooperation, a node may not want to borrow its server more often than the other node borrows its own one (recall the goal of a node is to cooperate without gain a net rewards). We call acceptance rate, $a_i$, the rate at which $n_i$ sees its server requests accepted. We have that
$$
a_1 = \lambda_1 p_2 \pi_{10} \: \: \: a_2 = \lambda_2 p_1 \pi_{01}
$$
so that a fair cooperation probability pair is any pair such that $a_1=a_2$, i.e.,
$$
p_2 = p_1 \frac{\pi_{01}}{\pi_{10}} \frac{\lambda_2}{\lambda_1}
$$
Interestingly (see later), it turns out that for any loads there is a (unique) Pareto efficient cooperation pair $(1,p^*_2)$ that is also fair, i.e., such that
$$
p^*_2 = \frac{\pi_{01}}{\pi_{10}} \frac{\lambda_2}{\lambda_1}
$$
Also, from the solution of the chain (see later), one finds that $a_1$ ($a_2$) decreases with $p_1$ ($p_2$). We can now answer to the original question. As the rates $a_i$ are both observable quantities from a node, a possible distributed algorithm that determines the cooperation probability can simply exploit a bisection search. A detailed description of the algorithm is given later in the paper. 

The algorithm works as following. Assume that the loads doesn't change during the estimation of $a$. The algorithm is organized in rounds and it is based on the bisection method. At beginning of a round a node observes the acceptance rates of previous round and changes the current cooperation probability, i.e., the acceptance rates are used as feedback for the next round. Rounds are executed until $r=\frac{a_i}{a_j}<1-\epsilon$

At the first round of the algorithm, both nodes set $p_i=1$ (no observations are possible). If $\lambda_2=\lambda_1$ the algorithm terminates. Otherwise, assuming that $\lambda_2<\lambda_1$,
we now that $p^*_1=1,p^*_2<1$. Now, with this loads, $a_1>a_2$, hence $r_1>1$. According to the algorithm, $n_1$ keeps $p_1=1$, while $n_2$ uses a bisection search to determine an estimation of $p^*_2$: $n_2$ uses the interval $I=[x,y]$,  where initially $x=0,y=1$ and  $I$ is updated such that $p^*_2 \in I$. 
At the beginning of a round, $n_2$ sets $p_2=\frac{x+y}{2}$. If $r_2 \in [1-\epsilon,1+\epsilon]$ the algorithm terminates. Otherwise, if $r_2<1-\epsilon$, $n_2$  updates the upper limit of the interval, $y=p_2$, otherwise $r_2>1-\epsilon$ and $n_2$ updates the lower limit, $x=p_2$. It then sets $p_2=\frac{x+y}{2}$. Clearly, the new interval contains $p^*_2$, and it is shorter. So the termination condition is eventually reached.


\section{Property of cooperation (formal results)}
To proof the key properties of the 2-nodes,1-server model, we solve the Markov chain in Figure \ref{fig:MC} and analyze the corresponding expression of the blocking probabilities.
The computation of the steady state probability $\pi_{ij}$ of state $(i,j)$, boils down to solve the linear system of equations:
%\scriptsize
$$
  -a & 1 & 1 & 0 \\
 \begin{bmatrix} 
  \lambda_1 & -b   & 0 & 1 \\
  \lambda_2 & 0 & -c   & 1 \\
  1 & 1 & 1 & 1 
 \end{bmatrix}
 \times \left[ \begin{array}{c} \pi_{00} \\ \pi_{10} \\ \pi_{01} \\ \pi_{11} \end{array} \right]  = \left[ \begin{array}{c} 0 \\ 0 \\ 0 \\ 1 \end{array} \right]
$$
%\normalsize
where, $a=\lambda_1+\lambda_2,b=1+\lambda_1+p_1\lambda_2,c=1+\lambda_2+p_2\lambda_1$.  Let $\mathbf{p}=(p_1,p_2)$ a cooperation probability pair.
\begin{definition}[Convenience] A cooperation pair $\mathbf{p}$ is convenient if
\[
b_1(\lambda_1,\lambda_2;\mathbf{p}) < \frac{\lambda_1}{1+\lambda_1}
\]
\[b_2(\lambda_1,\lambda_2;\mathbf{p}) < \frac{\lambda_2}{1+\lambda_2}
\]
\end{definition}
\begin{definition}[Pareto improvement]
A cooperation pair $\mathbf{p'}$ is a Pareto improvement w.r.t $\mathbf{p}$, if  $$b_i(\lambda_1,\lambda_2,\mathbf{p'})<b_i(\lambda_1,\lambda_2,\mathbf{p})$$ 
and 
$$b_j(\lambda_1,\lambda_2,\mathbf{p'}) \le b_j(\lambda_1,\lambda_2,\mathbf{p})
$$
where $i,j=1,2$.
\end{definition}
\begin{definition} [Efficient Convenient cooperation set]
A cooperation pair $\mathbf{p}$ is efficient and convenient if doesn't exit any other pair that is a Pareto improvement wrt to $\mathbf{p}$ and $\mathbf{p}$ is a convenient pair. $\partial P$ denotes the set of efficient and convenient pairs.
\end{definition}
\begin{definition} [Fair cooperation pair]
A cooperation pair $\mathbf{p}$ is fair if
$$
a_1(\mathbf{p}) =a_2 (\mathbf{p}) 
$$
\end{definition}

\begin{property}
The Efficient Convenient set is
$$
\partial P = \{(1,p)| p' \le p \le 1\} \cup \{(p,1)| p' \le p \le 1\}
$$
if $\lambda_2 \le \lambda^c_1$ or
$$
\partial P = \{(1,p)| 0 < p' \le p < 1\}
$$
otherwise
\\
\end{property} 
{\bf Proof}
The blocking probability can be rewritten as:
\begin{eqnarray*}
b_1(p_1,p_2)&=&\frac{(\kappa_1+\beta_1p_2)+(\alpha_1+\gamma_1p_2)p_1}{(\kappa+\beta p_2)+(\alpha+\gamma p_2)p_1}
\\
&=&\frac{(\kappa_1+\alpha_1p_1)+(\beta_1+\gamma_1p_1)p_2}{(\kappa+\alpha p_1)+(\beta+\gamma p_1)p_2}
\end{eqnarray*}
we have:
\begin{eqnarray*}
\frac{\partial b_1}{\partial p_1} &=& \frac{(\alpha_1+\gamma_1p_2)(\kappa+\beta p_2)-(\alpha+\gamma p_2)(\kappa_1+\beta_1p_2)}{(\kappa +\alpha p_1+\beta p_2+\gamma p_1p_2)^2}
\end{eqnarray*}
the denominator is positive, while the numerator is
$$        \lambda_2 (2 \lambda_2 + ...) 
  (2  +... - p_2 - \lambda_2 p_2)>0
$$
similarly
$$
\frac{\partial b_1}{\partial p_2} = \frac{(\beta_1+\gamma_1p_1)(\kappa+\alpha p_1)-(\beta+\gamma p_1)(\kappa_1+\alpha_1p_1)}{(\kappa +\alpha p_1+\beta p_2+\gamma p_1p_2)^2}
$$
where the numerator is
$$
- (2 \lambda_1 + \lambda_1^2 + ..)(2 + 3 \lambda_1 +..)<0
$$
Now, the two gradients $
\nabla b_1 = (\frac{\partial b_1 }{\partial p_1},\frac{\partial b_1 }{\partial p_2}),
\nabla b_2 = (\frac{\partial b_2 }{\partial p_1},\frac{\partial b_2 }{\partial p_2})
$
are not orthogonal since $\nabla b_1 \cdot \nabla b_2 <0$ and they both have a positive component. Hence, a Pareto improvement exits for any $p_1,p_2 < 1$, see Figure \ref{fig:IMPROVE}.

By requiring that the pair must be convenient we conclude the proof.

%\begin{property} [Limiting cooperation]
%p''_2=\frac{(\lambda_1+\lambda^2_1)(2+\lambda_1+\lambda_2)}{\lambda_2(\lambda_2+\lambda_2\lambda_1+\lambda^2_2-\lambda_1)}
%$$
%p'_2=\frac{\lambda_2(2+\lambda_1+\lambda_2)}{       2 \lambda_1+3\lambda^2_1+\lambda^3_1+2\lambda_1 \lambda_2+\lambda^2_1 \lambda_2+\lambda^2_2}
%$$
%$$
%$$
%\end{property}


\begin{property}
[Fair optimal cooperation] The fair  cooperation pair is optimal
\end{property}
{\bf Proof} 
Solving the MC with the additional constrain $\lambda_1 \pi_{10} p_2= \lambda_2 \pi_{01}$ provides $$
p^*_2=\Big(\frac{\lambda_2}{\lambda_1}\Big)^2
$$ since $p'_2<p_2<p''_2$ the property holds. 


\subsection{K-servers,2-providers Model}


% $$
% \nabla b_1 = (\frac{\partial b_1}{\partial p_1},\frac{\partial b_1}{\partial p_2}) \:\: \nabla b_2  = (\frac{\partial b_2}{\partial p_1},\frac{\partial b_2}{\partial p_2})
% $$ We will show that for every pair $p'=(p'_1,p'_2) \notin P^*$, it there exits a vector $v=(v_1,v_2), v_1,v_2>0$, such that $(\nabla b_1 \cdot v)_{p=p'} < 0, (\nabla b_2 \cdot v)_{p=p'} <0$.

 In this case, to determine the set of loads for which cooperation is convenient, we can use the Erlang-B formula that for just one or two servers is $\frac{\la a_2 = \pi_{01} p_1 \lambda_2mbda}{1+\lambda}$ and $\frac{\lambda^2}{2+2\lambda+\lambda^2}$ respectively. Assuming $\lambda_1 > \lambda_2$, for cooperation to be convenient for both nodes, it must be:
$$
\frac{(\lambda_1+\lambda_2)^2}{2+2(\lambda_1+\lambda_2)+(\lambda_1+\lambda_2)^2} < \frac{\lambda_2}{1+\lambda_2}
$$ 
After some manipulation one finds the critical value indicating the minimum $\lambda_2$ for which cooperation is convenient: (see also Figure \ref{fig:CONV})
\begin{equation}
\lambda_2 > \lambda^c_1 = \sqrt{1+\lambda_1}-1
\label{equ:LOAD_CONV}
\end{equation}

\begin{figure}[ht] 
    \centering
  \includegraphics[width=0.48\linewidth]{eps/cross} 
    %\vspace{4ex}
\caption{Cooperation convenience}
\label{fig:CONV} 
\end{figure}%% 

As role of thumb $\lambda^c=\frac{\lambda}{2}. $We now will show that when nodes cooperate with a certain probability, cooperation can be made convenient for arbitrary loads. Before that, it is worth to analyze why use probability at all.
Deterministic rules to regulate cooperation fail


To understand the effect of the cooperation probabilities, Figure \ref{fig:PARETO_095095} shows $b_1()$ and $b_2()$ for $\lambda_1=\lambda_2=0.95$ as a function of the cooperation probabilities and two contour lines on the $p_1 \times p_2$ domain, one for $b_1(p_1,p_2)=b_1(0,0)$ (bottom line) and the other for $b_2(p_1,p_2)=b_2(0,0)$, that divide the domain $[0,1]^2$ into two parts. A domain $P$ where the blocking probability is lower the two nodes at the same time, labelled OK, and the remaining part where one of the two nodes has a higher blocking probability. The two arrows point to the direction where the decrease in the blocking probability is maximum, see later.
\begin{figure}[ht] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering    \includegraphics[width=0.99\linewidth]{eps/pareto12_095095}
    \label{fig:P12_095}
    \caption{Cooperation probability effect}
    %\vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso095095}       
  \caption{Cooperation domains}
  \label{fig:DOMAIN_095095} 
  \end{subfigure}
\caption{Blocking probabilities vs cooperation probabilities, for $\lambda_1=\lambda_2=0.95$}
\label{fig:PARETO_095095}
\end{figure}
The next two figures show that $P$, when $\lambda_2<\lambda_1$ is not empty and, in particular, this also occurs when loads violate the condition expressed by Equation \ref{equ:LOAD_CONV}. Figure \ref{fig:PARETO_09504} shows the blocking probabilities and cooperation domains for $\lambda_1=0.4,\lambda_2=0.95,$, i.e., $\lambda_2>\sqrt{\lambda_1+1}-1$, whereas Figure for $\lambda_1=0.4,\lambda_2=0.25,$, i.e., $\lambda_2<\sqrt{\lambda_1+1}-1$

\begin{figure}[ht] 
  \centering
    \begin{subfigure}[b]{0.5\linewidth}
  \includegraphics[width=0.99\linewidth]{eps/pareto12_09504} 
    \caption{Blocking probabilities} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso09504}
    \caption{Cooperation domains} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
    \caption{Blocking probabilities for $\lambda_1=0.95,\lambda_2=0.4$}
    \label{fig:PARETO_09504} 
\end{figure}


\begin{figure}[ht] 
  \centering
    \begin{subfigure}[b]{0.5\linewidth}
  \includegraphics[width=0.99\linewidth]{eps/pareto12_095025} 
    \caption{Blocking probabilities} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/iso095025}
    \caption{Cooperation domains} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
    \caption{Blocking probabilities for $\lambda_1=0.95,\lambda_2=0.25$}
    \label{fig:PARETO_095025} 
\end{figure}

\subsection{Optimum way to cooperate} Q2) Is there exits a cooperation probability pair that minimizes the blocking probabilities for both nodes? To answer to this question, it is useful to first considering the problem of minimizing the blocking probabilities as a multi-objectives minimization problem 
$$
min [b_1(\mathbf{p}),b_2(\mathbf{p})] \:\:\:\: \mathbf{p} \in [0,1]^2
$$
where $\mathbf{p}=(p_1,p_2)$. Note that in our problem we additional require that $b_1(\mathbf{p})<b_1(0),b_2(\mathbf{p})<b_2(0)$.

We can now use the notion of Pareto efficiency. For a given a cooperation probability pair, $\mathbf{p}$, $\mathbf{p}'$ is a Pareto improvement wrt $\mathbf{p}$, if $b_1(\mathbf{p}')<b_1(\mathbf{p})$ and $b_2(\mathbf{p}') \leq b_2(\mathbf{p})$ or $b_2(\mathbf{p}')<b_2(\mathbf{p})$ and $b_1(\mathbf{p}') \leq b_1(\mathbf{p})$, i.e., with the new solution at least one blocking probability is lower than the old one. Also, $\mathbf{p}^*$ is said to be Pareto efficient (or optimal) if it doesn't exit any Pareto improvement   wrt to $\mathbf{p}^*$. The set of pairs that are Pareto optimal is called the set of efficient solutions, $\partial P$, and the corresponding  image through the $\mathbf{b}=(b_1,b_2)$  function, the Pareto frontier, $\partial B$, i.e., $\partial B = \mathbf{b}(\partial P)$. So the answer to the original question is that the optimal cooperation probability pair is any pair in the $\partial P$ set and such that $b_1(\mathbf{p})<b_1(0),b_2(\mathbf{p})<b_2(0)$%As we also want that for the two nodes the blocking probability under cooperation should be less than they do not cooperate
Figure \ref{fig:IMAGE} shows an example of the Pareto frontier for $\lambda_1=\lambda_2=0.95$. 


\begin{figure}[ht] 
\centering
  \includegraphics[width=0.7\linewidth]{eps/image} 
    \label{fig:IMAGE} 
    \caption{An example of Image of the b function for $\lambda_1=\lambda_2=0.9$. The two solid lines is the (convenient) Pareto frontier; dashed lines represent the border after which cooperation is not convenient for one of the two nodes.} 
    \label{fig:FRONTIERA} 
\end{figure}




\subsection{Reaching optimum cooperation} Q3) How the two nodes can agree on determining such optimal cooperation probabilities using a distributed algorithm? First of all, we know that there are many Pareto efficient probability cooperation pairs, and that, assuming $\lambda_2 < \lambda_1$, their form is $(1,p_2)$, with $p_2 \le 1$. In principle, any of them is a convenient choice. However, an additional reasonable criteria to seek among these probabilities is to require that the rate at which $n_1$ borrows its server to $n_2$ is to be equal to the rate at which $n_2$ borrows its server to $n_1$. We call this requirement {\it fair} cooperation. Although convenient wrt to cooperation, a node may not want to borrow its server more often than the other node borrows its own one (recall the goal of a node is to cooperate without gain a net rewards). We call acceptance rate, $a_i$, the rate at which $n_i$ sees its server requests accepted. We have that
$$
a_1 = \lambda_1 p_2 \pi_{10} \: \: \: a_2 = \lambda_2 p_1 \pi_{01}
$$
so that a fair cooperation probability pair is any pair such that $a_1=a_2$, i.e.,
$$
p_2 = p_1 \frac{\pi_{01}}{\pi_{10}} \frac{\lambda_2}{\lambda_1}
$$
Interestingly (see later), it turns out that for any loads there is a (unique) Pareto efficient cooperation pair $(1,p^*_2)$ that is also fair, i.e., such that
$$
p^*_2 = \frac{\pi_{01}}{\pi_{10}} \frac{\lambda_2}{\lambda_1}
$$
Also, from the solution of the chain (see later), one finds that $a_1$ ($a_2$) decreases with $p_1$ ($p_2$). We can now answer to the original question. As the rates $a_i$ are both observable quantities from a node, a possible distributed algorithm that determines the cooperation probability can simply exploit a bisection search. A detailed description of the algorithm is given later in the paper. 

The algorithm works as following. Assume that the loads doesn't change during the estimation of $a$. The algorithm is organized in rounds and it is based on the bisection method. At beginning of a round a node observes the acceptance rates of previous round and changes the current cooperation probability, i.e., the acceptance rates are used as feedback for the next round. Rounds are executed until $r=\frac{a_i}{a_j}<1-\epsilon$

At the first round of the algorithm, both nodes set $p_i=1$ (no observations are possible). If $\lambda_2=\lambda_1$ the algorithm terminates. Otherwise, assuming that $\lambda_2<\lambda_1$,
we now that $p^*_1=1,p^*_2<1$. Now, with this loads, $a_1>a_2$, hence $r_1>1$. According to the algorithm, $n_1$ keeps $p_1=1$, while $n_2$ uses a bisection search to determine an estimation of $p^*_2$: $n_2$ uses the interval $I=[x,y]$,  where initially $x=0,y=1$ and  $I$ is updated such that $p^*_2 \in I$. 
At the beginning of a round, $n_2$ sets $p_2=\frac{x+y}{2}$. If $r_2 \in [1-\epsilon,1+\epsilon]$ the algorithm terminates. Otherwise, if $r_2<1-\epsilon$, $n_2$  updates the upper limit of the interval, $y=p_2$, otherwise $r_2>1-\epsilon$ and $n_2$ updates the lower limit, $x=p_2$. It then sets $p_2=\frac{x+y}{2}$. Clearly, the new interval contains $p^*_2$, and it is shorter. So the termination condition is eventually reached.


\section{Property of cooperation (formal results)}
To proof the key properties of the 2-nodes,1-server model, we solve the Markov chain in Figure \ref{fig:MC} and analyze the corresponding expression of the blocking probabilities.
The computation of the steady state probability $\pi_{ij}$ of state $(i,j)$, boils down to solve the linear system of equations:
%\scriptsize
$$
  -a & 1 & 1 & 0 \\
 \begin{bmatrix} 
  \lambda_1 & -b   & 0 & 1 \\
  \lambda_2 & 0 & -c   & 1 \\
  1 & 1 & 1 & 1 
 \end{bmatrix}
 \times \left[ \begin{array}{c} \pi_{00} \\ \pi_{10} \\ \pi_{01} \\ \pi_{11} \end{array} \right]  = \left[ \begin{array}{c} 0 \\ 0 \\ 0 \\ 1 \end{array} \right]
$$
%\normalsize
where, $a=\lambda_1+\lambda_2,b=1+\lambda_1+p_1\lambda_2,c=1+\lambda_2+p_2\lambda_1$.  Let $\mathbf{p}=(p_1,p_2)$ a cooperation probability pair.
\begin{definition}[Convenience] A cooperation pair $\mathbf{p}$ is convenient if
\[
b_1(\lambda_1,\lambda_2;\mathbf{p}) < \frac{\lambda_1}{1+\lambda_1}
\]
\[b_2(\lambda_1,\lambda_2;\mathbf{p}) < \frac{\lambda_2}{1+\lambda_2}
\]
\end{definition}
\begin{definition}[Pareto improvement]
A cooperation pair $\mathbf{p'}$ is a Pareto improvement w.r.t $\mathbf{p}$, if  $$b_i(\lambda_1,\lambda_2,\mathbf{p'})<b_i(\lambda_1,\lambda_2,\mathbf{p})$$ 
and 
$$b_j(\lambda_1,\lambda_2,\mathbf{p'}) \le b_j(\lambda_1,\lambda_2,\mathbf{p})
$$
where $i,j=1,2$.
\end{definition}
\begin{definition} [Efficient Convenient cooperation set]
A cooperation pair $\mathbf{p}$ is efficient and convenient if doesn't exit any other pair that is a Pareto improvement wrt to $\mathbf{p}$ and $\mathbf{p}$ is a convenient pair. $\partial P$ denotes the set of efficient and convenient pairs.
\end{definition}
\begin{definition} [Fair cooperation pair]
A cooperation pair $\mathbf{p}$ is fair if
$$
a_1(\mathbf{p}) =a_2 (\mathbf{p}) 
$$
\end{definition}

\begin{property}
The Efficient Convenient set is
$$
\partial P = \{(1,p)| p' \le p \le 1\} \cup \{(p,1)| p' \le p \le 1\}
$$
if $\lambda_2 \le \lambda^c_1$ or
$$
\partial P = \{(1,p)| 0 < p' \le p < 1\}
$$
otherwise
\\
\end{property} 
{\bf Proof}
The blocking probability can be rewritten as:
\begin{eqnarray*}
b_1(p_1,p_2)&=&\frac{(\kappa_1+\beta_1p_2)+(\alpha_1+\gamma_1p_2)p_1}{(\kappa+\beta p_2)+(\alpha+\gamma p_2)p_1}
\\
&=&\frac{(\kappa_1+\alpha_1p_1)+(\beta_1+\gamma_1p_1)p_2}{(\kappa+\alpha p_1)+(\beta+\gamma p_1)p_2}
\end{eqnarray*}
we have:
\begin{eqnarray*}
\frac{\partial b_1}{\partial p_1} &=& \frac{(\alpha_1+\gamma_1p_2)(\kappa+\beta p_2)-(\alpha+\gamma p_2)(\kappa_1+\beta_1p_2)}{(\kappa +\alpha p_1+\beta p_2+\gamma p_1p_2)^2}
\end{eqnarray*}
the denominator is positive, while the numerator is
$$        \lambda_2 (2 \lambda_2 + ...) 
  (2  +... - p_2 - \lambda_2 p_2)>0
$$
similarly
$$
\frac{\partial b_1}{\partial p_2} = \frac{(\beta_1+\gamma_1p_1)(\kappa+\alpha p_1)-(\beta+\gamma p_1)(\kappa_1+\alpha_1p_1)}{(\kappa +\alpha p_1+\beta p_2+\gamma p_1p_2)^2}
$$
where the numerator is
$$
- (2 \lambda_1 + \lambda_1^2 + ..)(2 + 3 \lambda_1 +..)<0
$$
Now, the two gradients $
\nabla b_1 = (\frac{\partial b_1 }{\partial p_1},\frac{\partial b_1 }{\partial p_2}),
\nabla b_2 = (\frac{\partial b_2 }{\partial p_1},\frac{\partial b_2 }{\partial p_2})
$
are not orthogonal since $\nabla b_1 \cdot \nabla b_2 <0$ and they both have a positive component. Hence, a Pareto improvement exits for any $p_1,p_2 < 1$, see Figure \ref{fig:IMPROVE}.

By requiring that the pair must be convenient we conclude the proof.

%\begin{property} [Limiting cooperation]
%p''_2=\frac{(\lambda_1+\lambda^2_1)(2+\lambda_1+\lambda_2)}{\lambda_2(\lambda_2+\lambda_2\lambda_1+\lambda^2_2-\lambda_1)}
%$$
%p'_2=\frac{\lambda_2(2+\lambda_1+\lambda_2)}{       2 \lambda_1+3\lambda^2_1+\lambda^3_1+2\lambda_1 \lambda_2+\lambda^2_1 \lambda_2+\lambda^2_2}
%$$
%$$
%$$
%\end{property}


\begin{property}
[Fair optimal cooperation] The fair  cooperation pair is optimal
{\bf Proof} 
\end{property}
Solving the MC with the additional constrain $\lambda_1 \pi_{10} p_2= \lambda_2 \pi_{01}$ provides $$
p^*_2=\Big(\frac{\lambda_2}{\lambda_1}\Big)^2
$$ since $p'_2<p_2<p''_2$ the property holds. 



\subsection{K-servers,2-providers Model}


% $$
% \nabla b_1 = (\frac{\partial b_1}{\partial p_1},\frac{\partial b_1}{\partial p_2}) \:\: \nabla b_2  = (\frac{\partial b_2}{\partial p_1},\frac{\partial b_2}{\partial p_2})
% $$ We will show that for every pair $p'=(p'_1,p'_2) \notin P^*$, it there exits a vector $v=(v_1,v_2), v_1,v_2>0$, such that $(\nabla b_1 \cdot v)_{p=p'} < 0, (\nabla b_2 \cdot v)_{p=p'} <0$.


==> algorithm.tex <==

In this section, we propose a distributed algorithm running at the fog nodes to determine the optimal cooperation probability vector for each fog node. The algorithm leverages the cooperation ratios $r_j$ measured locally at each node $n_j$, defined as $r_j = \frac{R^{in}_j}{R^{out}_j}$


A convenient alternative to express the condition $R^{in}_j=R^{out}_j$ is $r_j=1$, both result in checking fairness using an estimation of the two flows. We first describe a centralized algorithm to solve the minimization problem $\cP$ on the light of our previous findings, where $r_j$ is computed using the N-$MC$ model.
Then propose a distributed protocol implementing the algorithm where $r_j$ is estimated at run-time. 



\subsection{Centralized Algorithm}
The key idea behind our algorithm is that the minimization problem $\cP$ (Eq.~\ref{prolem:min}) using the N-$MC$ model can be reduced to the problem of finding the zero of the following function:
\begin{equation}
\label{equ:zero}
g(\mathbf{p}) = \sum_{j=2}^N |1 - r_j(\mathbf{p})|   \:\:\:  \mathbf{p} \in \{1\} \times (0,1]^{N-1}
\end{equation}
%where 
%$$
%f_j(\mathbf{p}) = |1 - r_j(1,\mathbf{p})|
%$$
This function has a unique zero when the argument is $\mathbf{p}^*$. In fact, if two zeros were possible, this means that it there exists two cooperation probability vectors $(1,p^*_2,\ldots,p^*_N)$ and $(1,p^{*'}_2,\ldots,p{*'}_N)$, which contradicts our results obtained in Section \ref{sec:OPT_NUM}. 

The basic idea of the algorithm is to
find the zero of $g$ by sequentially selecting a suitable $j$ and finding the cooperation probabilities that makes $r_j \sim 1$. This operation is repeated until all $r_j \sim 1$ or a maximum number of iterations is reached. 


(a) {\it how to select $j$?}: The index $j$ is selected in a way that the $r_j \sim 1$ can be reached by only changing $p_j$ and keeping the other $p_i$ fixed. This property will allow to implement the algorithm in a distributed way (see later). To ensure that this can be obtained, $j$ must be such that $r_j>1$. In fact, suppose that for a given $\mathbf{p}$, with $p_j=p'_j>0$, $r_j(\mathbf{p})>1$. From Eq. \ref{equ:accept}, we see that if $p_j=0$ then $R^{in}_j=0$, \ie $r_j(\mathbf{p'})=0$, where $\mathbf{p}=\mathbf{p}$, but the $j$-th component set to 0. Now, it is reasonable to assume that $r_j$ is a monotonic function of $p_j$, so that a unique value $p^*_j, p_j<p^*_j<0$ such that $r_j=1$ should exist. When more indexes exit with $r_j>1$, the algorithm selects $j$ whose $r_j$ is maximum, as it provides the highest contribution to the $g$; Alg.~\ref{algo:optimal_centralized} provides these steps in a more formal way.


(b) {\it how to find $p^*_j$?}: To compute $p^*_j$ we leverage a bisection algorithm for its robustness compared to convergence





%Alg.~\ref{algo:optimal_centralized}  






\begin{algorithm}[!t]
\scriptsize
\caption{Cooperation Probabilities
\label{algo:optimal_centralized}}
%\scriptsize
%\textbf{Init:} $[a_j,b_j]\gets$ [0,1]
\textbf{Input:} $Steps, \epsilon$\\
\textbf{Output:} $\mathbf{p}$
\begin{algorithmic}[1]
%\State Warm-up
\State $\mathbf{p} \gets \mathbf{1}$
\State $\mathbf{r} \gets$ Compute\_Ratios($\mathbf{p}$)
%\State $j \gets \{ i, \max(r_i>1)\}$
\State $j \gets$  argmax$_i$ $\{r_i \ge 1+\epsilon\}$
\While {$j \ne null \And Step>0$ } 
\State $\mathbf{p}_j \gets $ Bisection($j$)
\State $\mathbf{r} \gets$ Compute\_Ratios($\mathbf{p}$)
%\State $j \gets \{i, \max(r_i>1)\}$
\State $j \gets$  argmax$_i$ $\{r_i \ge 1+\epsilon\}$
\State $Step \gets Step - 1$
\EndWhile
\end{algorithmic}
\end{algorithm}



Alg.~\ref{algo:optimal_centralized}  first computes the cooperation ratios $r_j$ for $\mathbf{p}=\mathbf{1}$. It then selects the node $j$ with the maximum $r_j>1+\epsilon$, where $\epsilon$ is an allowed approximation error, and call a bisection search algorithm on the selected node $j$. These steps are repeated until no nodes can be selected or the maximum allowed number of cycles is reached.

%The bisection search algorithm (Algorithm \ref{alg:coop}) tunes the cooperation probability $p_j$ in $\mathbf{p}$ until  $|1-r_j(\mathbf{p})| \le \epsilon$. Note that $r_j>1$ means that the node $j$ is accepting more tasks than what the other nodes are currently accepting. Hence, to reduce $r_j$, $p_j$ has to be decreased.



%\begin{algorithm}[!t]
%\caption{\label{alg:coop} Bisection Search For Node $j$}
%\scriptsize
%\textbf{Input:} $j,\epsilon$\\
%\textbf{Output:} $p_j$
%\begin{algorithmic}[1]
%\State $[min_j,max_j] \gets [0,1]$
%\State $p_j \gets \frac{min_j+max_j}{2}$
%\State $p_j \gets 1$
%\State $r_j \gets$ Compute\_Ratio($j$)
%\While {$|1-r_j| > \epsilon$} 
%\If{$r_j>1$} \Comment{decrease cooperation probability}
%\State $max_j \gets p_j$ \Comment{decrease upper limit}
%\Else \Comment{increase cooperation probability}
%\State $min_j \gets p_j$ \Comment{increase lower limit}
%\EndIf
%\State $p_j \gets \frac{min_j+max_j}{2}$
%\State $r_j \gets$ Compute\_Ratio($j$)
%\EndWhile
%\end{algorithmic}
%\end{algorithm}




We run the proposed algorithm on a sample network of four fog nodes, and report the execution rounds of this algorithm in Table~\ref{table:round}.
%Figure \ref{fig:tuning} shows a trace of the algorithm.


\begin{table}[!t]
\scriptsize
\begin{center}
\begin{tabular}{|c|c|c|c|}
  \hline
   $n_1$ & $n_2$ & $n_3$ & $n_4$ \\ \hline \hline
   0.675 & 0.875 & 1.154 & {\bf 1.557} \\ \hline % 3
0.770 & 1.003 & {\bf 1.328 } & 0.994 \\ \hline % 2
0.850 & {\bf 1.111} & 1.006 & 1.084 \\ \hline % 1
0.884 & 1.010 & 1.042 & {\bf 1.121} \\ \hline % 3
0.911 & 1.040 & {\bf 1.072} & 0.999 \\ \hline % 2
0.934 & {\bf 1.065} & 0.995 & 1.019 \\ \hline % 1
0.963 & 0.991 & 1.022 & {\bf 1.045} \\ \hline % 3
0.975 & 1.003 & {\bf 1.034} & 0.993 \\ \hline % 2
0.983 & {\bf 1.011} & 1.009 & 0.999 \\ \hline % 1
0.988 & 0.999 & 1.003 &{\bf 1.013}   \\ \hline % 2
0.992 & 1.003 & 1.001 & 1.007 \\ \hline % 3
  \end{tabular}
\end{center}
\caption{.
Example of cooperation ratios  $r_j$ during the execution of Alg.~\ref{algo:optimal_centralized} for $N=4$ nodes, $\lambda_1=0.9,\lambda_1=0.8,\lambda_1=0.7$, and $\lambda_1=0.6$  with $\epsilon = 10^{-2}$. 
Bold values represent the next node running the bisection algorithm. Node IDs are reported in the first row.
} 
\label{table:round}
\end{table}


\subsection{Distributed Protocol}
We propose a candidate distributed protocol that tunes the cooperation probabilities based on the previous centralized algorithm. The protocol takes the following two considerations into accounts: (\textit{i}) when running the centralized algorithm we observed that the order with which nodes is selected is maintained over the iterations (see for example Table \ref{table:round}) and that this order reflects their loads (the values $r_j$ are inversionally proportional to the loads). The distributed protocol exploits this observation to implement a token circulating on a logical ring formed at the beginning the algorithm, where nodes are ordered according to their $r$ ; (\textit{ii}) the cooperation ratio is an approximation of the ideal ratio, hence subject to noise with false positives and negatives. To ensure that the bisection algorithm terminates a condition on the length of the current interval $[max-min]$ is added (see the next Section for additional details).

Our distributed algorithm, depicted in Alg.~\ref{algo:distributed}, operates as follows. We assume that nodes are connected and can communicate with each other. The algorithm is triggered by any node initiator, say $u$. An initiator node $u$ triggers the algorithm if: (\textit{i}) $u$ decides to cooperate in order to reduce its blocking probability (if nodes do not cooperate), or (\textit{ii}) $u$ decides to change the current cooperation probabilities (\eg if it detects a change in the current cooperation ratio). The algorithm consists of a {\it warm-up} phase and $R$ {\it tuning rounds}. Node $u$ sends a broadcast (\textit{bcast}) message to all the other nodes indicating a warm-up phase of the cooperation algorithm is going to be started. This phase lasts for a given time, $\Delta T$, specified in the message. 

Any node $j$, receiving this message, sets its cooperation probability to $p_j=1$ for the $\Delta T$ time interval. During this interval, $j$ measures the number of tasks received from other nodes for local execution at $j$, $in_j$ and the number of tasks that $j$ has sent for remote execution at other fog nodes $j'\neq j$, $out_j$. At the end of this warm-up phase, every node $j$ sends a reply message carrying $r_j=\frac{in_j}{out_j}$ to $u$. After receiving all the replies from the nodes, node $u$ creates a sorted list $s$ of nodes according to their values $r_j$, with the top ranked being the node with the highest $r_j$, expect the lowest one. This because the node with the lowest $r_j$ has to keep $p_j=1$ (this condition reflects the form of $\mathbf{p}^*$ discussed in Sect. \ref{sec:OPT_NUM}); also this order reflects the loads at the fog nodes. Node $u$ then creates a token message with this sorted list and an integer $R$. The message loops through the ring of nodes following the order in $s$, performing $R$ rounds. The token represents the right of a node to change its cooperation probability using a bisection algorithm. To estimate $r_j$ in the future, node $j$ uses two counters, $in_j$ and $out_j$. The value $r_j=\frac{in_j}{out_j}$ is computed soon as either  $in_j$ or $out_j$ is equal to $k$, where $k$ is a protocol parameter. The owner of the token starts using $max_j=1,min_i=0$ and tunes its cooperation probability until either $r_j$ is (close to) 1, or $max_j-min_j<\epsilon$. This stopping condition is defined to take the possible estimation errors of $r$ into account. A more formal protocol description in given in Alg.~\ref{algo:distributed}.


\begin{algorithm}[!t]
\scriptsize
\caption{\label{alg:trigger} Bisection Search Running on Node $j$ \label{algo:distributed}}
%\scriptsize
%\textbf{Init:} $[a_j,b_j]\gets$ [0,1]
\begin{algorithmic}[1]
\State \textbf{On accepting a Task}:
\State $in_j \gets in_j+1$
\If{$in_j==k$} 
\State Tune()
\EndIf
\State \textbf{On sending a Task}:
\State $out_j \gets out_j+1$
\If{$out_j==k$} 
\State Tune()
\EndIf
\State \textbf{On Tune:}
\State $r_j \gets \frac{in_j}{out_j}$
\State $in_j,out_j \gets 0$ 
\If{($r_j \ge 1 + \epsilon) \And (max_j-min_j > \epsilon)$} 
\State $max_j \gets p_j$
\State $p_j \gets (max_j+min_j)\frac{1}{2}$
\State return
\EndIf
\If{$r_j \le 1 - \epsilon \And max_j-min_j > \epsilon$} 
\State $min_j \gets p_j$
\State $p_j \gets (max_j+min_j)\frac{1}{2}$
\State return
\EndIf
\If {not.Token.last}
\State $update\_Token()$
\State \textbf{Send\_To\_Next}(Token)
\EndIf
\end{algorithmic}
\end{algorithm}

{\it Reaction to load changes} We remark that in case of change in the load, the first node $n_j$ that estimates $r_j>\epsilon$ can trigger another round with the purpose of re-tuning the cooperation probabilities. If the round fails (this occurs when the most loaded node is no longer node $n_1$), $n_j$ can starts the cooperating algorithm from starting a new warm-up phase.

%%%%%%%%%%
%% N Nodes
%%%%%%%%%%%

%\begin{algorithm}[!t]
%\caption{\label{alg:tuneN} Tuning of N nodes, running at node $j$}
%\scriptsize

%\Require 
%\textbf{Input:} $P={p_i} | i \in %{\{1..N\}\setminus\{j\}}$ \\
%\textbf{Output:} $p_j$
%\begin{algorithmic}[1]
%\State Payoff$=(0)^{NxN}; rounds=0$
%\If{OnReceive($p_i$)}
%\State $rounds++$
%\State Compute($bp_t$,$FI$)
%\State Payoff$[i][j]\gets p_i$
%\State Payoff$[j][i]\gets bp_t$
%\If{$bp_t>bp_{t-1}$}
%\State ReduceAndSend($p_j$)
%\Else \State IncreaseAndSend($p_j$)
%\EndIf
%\If{$|bp_t - \max($Payoff$[j][x])_{x=1..N}| < \epsilon \And rounds > N $}
%\State \textbf{terminate}
%\ElsIf{ExpirationTime}
%\State $p_j=\max($Payoff$[j][x])_{x=1..N}$
%\State \textbf{terminate}
%\EndIf
%\EndIf
%\end{algorithmic}
%\end{algorithm}

==> fairness2.tex <==
\subsection{Fairness based on the Acceptance probability}
We say that the cooperation among nodes is fair, when all nodes have the same {\it acceptance probability}
The probability that a task of node $i$ is accepted by node $j$ is the probability that node $i$ is congested and node $j$ is idle
$$
Pr\{s_i=1,s_j=0, n_j \:\: accepts\} = \sum_{s: s_i=1,s_j=0} \pi_s \frac{p_j}{N-1}
$$
The probability $s_i$ is congested is
$$
Pr\{s_i=1\} = \sum_{s: s_i=1} \pi_s
$$
$$
Pr\{s_j=0, n_j \:\: accepts | s_i=1\} =\frac{Pr\{s_i=1,s_j=0, n_j \:\: accepts\}}{Pr\{s_i=1\}}
$$
there is an error in the acceptance probability definition. it must be: Prob $j$ accepts $i$ given $i$ is congested (independently if it $j$ is busy or not) 
Define the matrix
$$
A
$$
where
$$
a_{ij}= \frac{\sum_{s: s_i=1,s_j=0} \pi_s}{\sum_{s: s_i=1}\pi_s}
$$
and $a_ii=0$.
The acceptance probabilities can be expressed as a function of the cooperation probabilities as
$$
pa = A p
$$
Define the difference matrix
$$
D
$$
where 
$$
d_{ij}=-1 \:\: i=j, d_{ij}=1, j=(i+1)\%N
$$
we have
$$
D (A p) = (DA) p = F p
$$
is the difference acceptance probabilities. we want that this difference is zero:
$$
F p = 0
$$
in the fixed point algo, we compute the next p from
$$
p=F^{-1} [0|1]
$$
the second vector say: all zero but $p_1=1$. In the code this is called FixedPoint3

==> game_old.tex <==
\begin{table}
 \centering
    \begin{tabular}{*{4}{c|}}
      \multicolumn{2}{c}{} & \multicolumn{2}{c}{Node 2}\\\cline{3-4}
      \multicolumn{1}{c}{} &  & 0  & 1\\\cline{2-4}
      \multirow{2}*{Node 1}  & 0 & 52,52 & 71,43 \\\cline{2-4}
      & 1 & 43,71 & 63,63 \\\cline{2-4}
    \end{tabular}
      \caption{A numerical example of the payoff matrix}
  \label{tab:Payoff} 
\end{table}


\begin{table}
 \centering
    \begin{tabular}{*{6}{c|}}
      \multicolumn{2}{c}{} & \multicolumn{3}{c}{Node 2}\\\cline{3-5}
      \multicolumn{1}{c}{} &  & 0  & 0.5 & 1 \\\cline{2-5}
      \multirow{3}*{Node 1}  & 0 & 52.6,52.6 & 63.2,47.6 & 71.1,43.8 \\\cline{2-5}
      & 0.5 & 47.6,63.2 & 58.5,58.5 & 66.6,55.0  \\\cline{2-5}
      & 1 & 43.8,71.1 & 55.0,66.6 & 63.3,63.3  \\\cline{2-5}
    \end{tabular}
      \caption{A numerical example of the payoff matrix with 3 strategies}
  \label{tab:Payoff2} 
  \end{table}


% \subparagraph{Bounded budget, same price, same loads}
% In this case $A$ and $B$ have the same budget $B$. This means that $c(k)$ takes value in the range $[0,2B]$. In this case, we say that a cooperation miss event occurs when $A$ is congested and $c=0$.  
% Due to symmetry, the coin can increase or decrease with the same probability (since the cooperation requests occurs with the same frequency). When $c=0$ however, the next variation can only be an increase. Similarly, when $c=2B$ the only variation possible is a decrease. In other words, $c(k)$ is a random walk on with reflecting barriers on $[0,2B]$. We can compute a lower bound  of the probability that a miss event occurs, $P_m$.

% A miss event occurs when $c=0$ the provider wants to buy a resource. In this case, the coin goes to state $c=-1$.. 




% Assume that a miss event is just occurred and that the next cooperation request is from $B$ to $A$ (this is why we are computing a lower bound). The average number of coin variations before the next miss event occurs is the expected return time to $0$, of the natural random walk starting from $c(0)=1$. This time is $4B+1$, .because...). Hence, $P_m=\frac{1}{4B+1}$.



% \subparagraph{Bounded budget, same price, different loads}
% In this case $A$ and $B$ have the same initial budget, $B$. However, due to the difference in the loads the probability that $A$ requires a resource to $B$ is different of the probability that $B$ requires a resource to $A$. Let
% Pr\{e_{AB}\}=p, \:\:\:\: Pr\{e_{BA}\}=q=1-p
% $$
% $$
% In this case $P_{m_A} \ne P_{m_B}$ and both can be computed as the inverse of the return time. 



% \subparagraph{Bounded budget, different price, different loads }


%  \begin{figure}
%  \centering
%  \includegraphics[width=0.5\textwidth]{eps/MC}
%  \caption{\label{fig:MC} Dynamic of a coin.}
%  \end{figure}



==> otherResult.tex <==
\begin{figure}[ht] 
  \centering
    \begin{subfigure}[b]{0.5\linewidth}
  \includegraphics[width=0.99\linewidth]{eps/pareto1_09504} 
    \caption{.} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/pareto2_09504.eps}
    \caption{..} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/pareto12_09504.eps}
    \caption{..} 
    \label{fig:DOMAIN09504} 
    %\vspace{4ex}
  \end{subfigure}  
  
    \caption{Blocking probabilities for $\lambda_1=0.95,\lambda_2=0.4$}
    \label{fig:PARETO_09504} 
\end{figure}


\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Node  & 1  & 2  & 3  & 4  \\ \hline
NCoop [L|C] & 50.3 | 49.7 & 50.3 | 49.7 & 50.3 | 49.7 & 50.3 | 49.7  \\ \hline
Coop [L|C] & 39.1 | 38.5 & 39.1 | 38.5 & 39.1 | 38.5 & 39.1 | 38.5  \\ \hline   
\end{tabular}
\end{center}
\caption{Example of task execution location for the traffic profile S(0.99,1), Local vs Cloud } \label{table:repartition1}
\end{table}

\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Node  & 1  & 2  & 3  & 4  \\ \hline
NCoop [L|C] & 52.6 | 47.4 & 53.8 | 46.2 & 55.1 | 44.9 & 56.3 | 43.7  \\ \hline
Coop [L|C] & 43.2 | 36.9 & 44.7 | 35.4 & 46.1 | 34.0 & 47.6 | 32.6  \\ \hline   
\end{tabular}
\end{center}
\caption{Example of task execution location for the traffic profile S(0.9,1.05), Local vs Cloud } \label{table:repartition2}
\end{table}




\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
  \begin{tabular}{|c |c|c|c|c|c|c|c|c|}
    \hline
    Node & 1 & 2 & 3 & 4 & 5 & 6 & 7  & 8 \\ \hline
    S(0.9,1) & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 \\ \hline
     S(0.9,1.05) &    19.7 & 20.4 & 21.1 & 21.8 & 22.5 & 23.1 & 23.7 & 24.4  \\ \hline
     S(0.9,1.1) &  15.2 & 16.4 & 17.6 & 18.7 & 19.8 & 20.8 & 21.7 & 22.6 \\ \hline
     S(0.9,1.15) & 12.1 & 13.6 & 15.1 & 16.5 & 17.8 & 19.0 & 20.0 & 20.9\\ \hline
  \end{tabular}
\end{center}
\caption{Cloud bandwidth reduction, 8 nodes} \label{table:reduction8}
\end{table}

==> results.tex <==
In this section, we present experimental analysis consisting of numerical and simulation results to evaluate f2f cooperation among fog nodes. 

%{\it Numerical Results: }
\subsubsection{Protocol convergence}
Fig.~\ref{fig:tuning} shows a trace of the centralized algorithm (Alg.~\ref{algo:optimal_centralized}) measuring the cooperation probability tuning over time.

\begin{figure}[t] 
  \centering
    \begin{subfigure}[b]{0.45\linewidth}
  \includegraphics[width=1\linewidth]{eps/tune4.eps}
    \caption{Trace of four nodes} 
    \label{fig:P12_09504} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=1\linewidth]{eps/tune8.eps}
    \caption{Trace of eight nodes} 
    %\vspace{4ex}
  \end{subfigure}  
  \caption{Example of cooperation probability tuning, $\lambda_1=0.9$. The other loads are $\lambda_{i+1}-\lambda_{i}=0.1$ (4 nodes) or $\lambda_{i+1}-\lambda_{i}=0.05$ (8 nodes). }
    \label{fig:tuning} 
\end{figure}

Fig.~\ref{fig:tuning} shows the blocking probability for $N=4$ nodes (a) and $N=8$ nodes (b). Each step corresponds to a new cooperation probability. The highest load is set at node 1, $\lambda_1=0.9$; and $\lambda_{i+1} $>$ \lambda_{i}=0.1$. Node $n_4$ is the first selected node to reduce its cooperation probability $p_4$. Its bisection based tuning algorithm ends at $p_4 \approx 0.5$. Then Alg.~\ref{algo:optimal_centralized} selects node $n_3$, that sets $p_3 \approx 0.65$ and then node $n_2$. A new 'round' is then executed during which all the three nodes are selected again, in the same order, and their cooperation probabilities are further reduced. The protocol converged after 60 steps organized into four rounds. For $N=8$, in Fig.~\ref{fig:tuning}(b), where load difference is set to 0.05 to achieve larger variation, the protocol converged after 6 rounds and 160 steps in total. %In these experiments $\epsilon$ was as small as $\epsilon=10^{-5}$, which we think allows to reliably check the convergence property of the Algorithm.

Fig.~\ref{fig:tuning_trace} shows the results of the simulation using our distributed algorithm running on a $N=4$ node network. We vary the number of servers per node and plot the blocking probability over time for $K=1$ (a) and $K=10$ (b) servers. We set the Fog-to-Fog link communication rate at $54$ Mpbs and the latency uniformly distributed in $U[0.5,1.2]$. %Results are given in The estimation of the cooperating ratio was done every $k=5000$ tasks (either sent or received) with $\epsilon=10^{-2}$.
The distributed algorithm converges in only 50 steps compared to 60 steps for the centralized algorithm. The distributed algorithm uses $\delta P$ which helps the algorithm stabilize and converge faster. 
Moreover, we show that increasing the number of servers per nodes further reduces the convergence time. %This is mainly due to .... {\bf CAN'T FIND AN EXPLANATION FOR THIS PARTICULAR RESULT!!}


\begin{figure}[t] 
  \centering
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/simuTune4.eps}
    \caption{$K=1$ server per node} 
    \label{fig:tune_k1} 
    %\vspace{4ex}
  \end{subfigure}  
     \begin{subfigure}[b]{0.45\linewidth}
    \centering
  \includegraphics[width=0.99\linewidth]{eps/simuTune4_c.eps}
    \caption{$K=10$ servers per node} 
    \label{fig:tune_k10} 
    %\vspace{4ex}
  \end{subfigure}  
         \caption{A trace of the cooperation protocol tuning phase for $N=4$ nodes, $\lambda_1=0.9,\lambda_2=0.8,\lambda_3=0.7 \lambda_4=0.6,k=5000,\epsilon=\delta P = 10^{-2}$, $K=1$ (a) and $K=10$ (b). The theoretical fair cooperation probabilities for $K=1$ are $p_1=1,p_2=.77,p_3=.57,p_4=.4$. }
    \label{fig:tuning_trace} 
\end{figure}


\subsubsection{Quantitative Blocking Probability Gain}
We discuss the blocking probability gain, defined as the percentage reduction in the blocking probability compared to no cooperation, for $N=2,4$ and $N=8$ nodes. We set the cooperation among nodes to the optimal values given by the $N$-MC model. 
In particular, we consider a geometric load profile, $G(q)$, where the ratio among two  $\lambda_i$ and $\lambda_{i+1}$ is a constant $q$ with $\lambda_1=\lambda$. \eg $G(1.05)$ can be interpreted as: the load of node $n_1$ is $\lambda_1=0.9$, and the load of node $n_2$ is $\lambda_2=\frac{0.9}{1.05} \approx 0.875$, while the load of node $n_3$ is $\lambda_3=\frac{0.875}{1.05} \approx 0.833$, and so on. 


Tables~~\ref{table:reduction2}, ~\ref{table:reduction4}, and ~\ref{table:reduction8} report the numerical results for $N=2$, 4, and 8 nodes respectively. For $N=2$, the gain of node $n_1$ is maximum for equal loads at the two nodes. This gain decreases with the difference in the loads. The contrary applies to $n_2$. This is due to the fairness constraint ensuring that the mean number tasks sent by of $n_1$ for execution by $n_2$ must be equal to the number of tasks that $n_1$ executes for $n_2$. When $\lambda_1>\lambda_2$, tasks received by $n_1$ register low acceptance rates by $n_2$ than tasks from $n_2$ executed by $n_1$.%, exactly because the rate at which $n_1$ receives is higher than the $n_2$'s rate, while the task forwarding rate must be equal. 

\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
  \begin{tabular}{|l|c|c|c|}
  \hline
  Load & $n_1$ & $n_2$  \\ \hline
G(1) & 22.6 & 22.6 \\ \hline
G(1.05) & 21.3 & 23.5 \\ \hline
G(1.1) & 20.0 & 24.2 \\ \hline
G(1.15)  & 18.9 & 25.0 \\ \hline
\end{tabular}
\end{center}
\caption{Cooperation gain, $N=2$ nodes, $\lambda_1=0.9$. } \label{table:reduction2}
\end{table}


When the number of fog nodes increases, see Table~\ref{table:reduction4} for $N=4$ results, the gain measured at node $n_1$ is maximum when all nodes have the same loads, and decreases with $q$. This occurs because nodes $n_2,n_3,n_4$ are seen by $n_1$ as a single entity with an average load $\lambda_e=\frac{1}{3}(\lambda_2+\lambda_3+\lambda_4)=\frac{1}{3}(\frac{1}{q}+\frac{1}{q^2}+\frac{1}{q^2})\lambda_1<\lambda_1$, which decreases with $q$ and the previous considerations can be applied to $n_1$. The variation of the gain for the other nodes shows a similar correlation with the loads, with the exception of $n_4$ for which the gain is almost constant. 

%{\bf DOES IT MAKE SENSE TO MEASURE THE OVERALL GAIN AS THE AVERAGE OF ALL GAIN AT THE NODES? I want to add a sentence to compare the gain when nodes increases but I couldn't. Need to verify if it makes sense to consider the overall gain or not!}

%Node $n_4$
%so that the pre and hence the   another node Since these loads decrease with $q$, the $n_1$'s gain also decreases with $q$ [EXPLAIN WHY THE GAIN OF NODE $n_3$ INCREASES].





\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
  \begin{tabular}{|l|c|c|c|c|}
  \hline
  Load & $n_1$ & $n_2$ & $n_3$ & $n_4$ \\ \hline
G(1) & 25.4 & 25.4 & 25.4 & 25.4  \\ \hline
G(1.05) & 22.1 & 23.2 & 24.4 & 25.5  \\ \hline
G(1.1) & 19.3 & 21.4 & 23.5 & 25.5  \\ \hline
G(1.15) & 15.1 & 18.8 & 22.2 & 25.3 \\ \hline
\end{tabular}
\end{center}
\caption{Cooperation gain, $N=4$ nodes, $\lambda_1=0.9$.} \label{table:reduction4}
\end{table}

\begin{table}[!t]
\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
%\tiny
  \begin{tabular}{|l |c|c|c|c|c|c|c|c|p{1.1cm}}
    \hline
    Load & $n_1$ & $n_2$ & $n_3$ & $n_4$ & $n_5$ & $n_5$ & $n_7$ & $n_8$ \\ \hline
    G(1) & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 & 26.3 \\ \hline
     G(1.05) &    19.7 & 20.4 & 21.1 & 21.8 & 22.5 & 23.1 & 23.7 & 24.4  \\ \hline
     G(1.1) &  15.2 & 16.4 & 17.6 & 18.7 & 19.8 & 20.8 & 21.7 & 22.6 \\ \hline
     G(1.15) & 12.1 & 13.6 & 15.1 & 16.5 & 17.8 & 19.0 & 20.0 & 20.9\\ \hline
  \end{tabular}
\end{center}
\caption{Cooperation gain, $N=8$ nodes, $\lambda_1=0.9$.} \label{table:reduction8}
\end{table}

%\begin{table}[!t]
%\begin{center}
%  \begin{tabular}{ |c|p{7.3cm}|}
%  \begin{tabular}{|l|c|c|c|c|}
%  \hline
%  Node & $n_1$ & $n_2$ & $n_3$ & $n_4$ \\ \hline
%G(0.99,1) & 22.6 & 22.6 & 22.6 & 22.6  \\ \hline
%G(0.99,1.05) & 19.8 & 20.8 & 21.9 & 22.9  \\ \hline
%G(0.99,1.1) & 17.4 & 19.3 & 21.2 & 23.0  \\ \hline
%G(0.99,1.15) & 15.4 & 18.1 & 20.7 & 23.1 \\ %\hline
%\end{tabular}
%\end{center}
%\caption{Cooperation gain using eight nodes.} %\label{table:reduction4bis}
%\end{table}

\subsubsection{Number of Cooperating Nodes}
We now elaborate about a scenario with $N=3$ fog nodes with load $\lambda_1 \ge \lambda_2 \ge \lambda_3$ and consider the node $n_1$'s point of view. What is the best cooperation strategy for $n_1$?: is it more convenient for $n_1$ to cooperate only with $n_2$, say strategy $C_2$, with $n_3$ (strategy $C'_2$), or with both $n_2$ and $n_3$ (strategy $C_3$)?. To answer to this question, we run several numerical experiments and found that the answer depends on the values of loads. %In the particular case when all loads are the same, $C_3$ is better than $C_2$, they gain being 22.6 and 24.7, respectively. The reason is that with the same loads the cooperation probabilities are set to $p_i=1$, and the system behaves for $C_2$ like an M/M/2/2 queue and for $C_3$ as an M/M/3/3 queue. The blocking probability then decreases due to the beneficial effect of an increased number of servers (raising from $K=2$ to $K=3$). 
For example, for $\lambda_1=0.9,\lambda_2=0.85,\lambda_3=0.8$ under $C_2$ the gain $21.0$, under $C'_2$ $19.5$ and under $C_3$ $21.8$. However, when $\lambda_3=0.7$ the gain under $C_3$ decreases to $20.0$, hence $C_2$ is the best.


Hence, in general the most efficient cooperation probability for  a given node have to be different for the specific  cooperating node. The problem of determining such probabilities can be not trivial and it is left as a future work.







%\subsubsection{Cooperation Ratio Estimation}
%A reliable ratio estimation is fundamental for the distributed tuning protocol to work correctly, as the variation in the cooperation probability is based on such estimations. 
 
%Suppose that $p^*_j$ is the optimal cooperation probability at node $j$ (\ie which provides a near-unitary cooperation ratio), $p_j$ the current cooperation probability, $I_j=[min_j,max_j]$ the current interval of possible cooperating probability that $n_j$ can use to change $p_j$, see Alg. \ref{algo:distributed}, and $\hat{r}_j$ the estimated cooperation ratio.  If $p_j \ne p^*_j$, the algorithm considers $p_j$ an acceptable value if and only if 

%(i) $\hat{r}_j(p_j) \sim 1$, or 

%(ii) when due to previous wrong estimations the range $I_j$ was updated in a way that $p^*_j \notin I$. These events correspond to false positive and negative errors of the estimation $\hat{r}$. 
 
 
%Instead of performing estimation every fixed amount of time (which is hard to set for every load), the protocol estimates cooperation ratio every $k$ received or sent tasks. To check the effect of $k$ on the estimation performance, we run several experiments varying $k$ for $r=1$. Results for the frequency distribution are shown in Fig.~\ref{fig:r_vs_k}. As expected, the shape of the distribution becomes narrowed around $r=1$ with increasing values $k$. 

%, while the estimation errors depend on $\epsilon$. 


%\begin{figure}[ht] 
%  \centering
%     \begin{subfigure}[b]{0.45\linewidth}
%    \centering
%  \includegraphics[width=0.99\linewidth]{eps/e1000.eps}
%    \caption{$k=1000$} 
%    \label{fig:r_vs_k_1000} 
%  \includegraphics[width=0.99\linewidth]{eps/e5000.eps}
%    %\vspace{4ex}
%  \end{subfigure}  
%     \begin{subfigure}[b]{0.45\linewidth}
%    \centering
%    \caption{$k=5000$} 
%    \label{fig:r_vs_k_5000} 
    %\vspace{4ex}
%  \end{subfigure}  
%    \caption{Empirical frequency distribution of 500 estimations obtained with $N=2$ nodes, $\lambda_1=\lambda_2=0.9,K=1$ server. }
%    \label{fig:r_vs_k} 
%\end{figure}

%We plot in Fig.~\ref{fig:coop_Ratio} the cooperation estimation over time.  In the rest of the simulation experiments we set $\epsilon=\delta P =10^{-2},k=5000$.

%\begin{figure}[ht] 
%  \centering
%    \begin{subfigure}[b]{0.45\linewidth}
%  \includegraphics[width=1\linewidth]{eps/tune.eps}
%    \caption{$\lambda_1=\lambda_2=0.9$} 
%    %\vspace{4ex}
%  \end{subfigure}  
%     \begin{subfigure}[b]{0.45\linewidth}
%    \centering
%  \includegraphics[width=1\linewidth]{eps/tuneb.eps}
%    \caption{$\lambda_1=0.9,\lambda_2=0.7$} 
    %\vspace{4ex}
%  \end{subfigure}  
%  \caption{Example of Cooperation ratio estimations. Estimation is done every $k$ tasks}
%    \label{fig:coop_Ratio} 
%\end{figure}



%\subsubsection{Scenarios}
%Poisson traffic
%Uniform traffic
%Beta traffic



%Figure shows the cooperation probability tuning for the bisection algorithm. Loads change at each vertical line starting from (0.9,0.8) as following (precision is 1e-6)
%(0.95,0.8), l1 increases --> p2 decreases (A=0)
%(0.95,0.4), l2 decreases --> p2 decreases (A=0)
%(0.8,0.4), l1 decreases, but l1>l2, p2 increases 
%(0.8,0.7) l2 increases, but l1>l2, increase
%(0.4,07) l2 decreases, but l1<l2, resets




==> simulation.tex <==









